Dictionary learning for clustering on hyperspectral images

Dictionary learning and sparse coding have been widely studied as mechanisms for unsupervised feature learning. Unsupervised learning could bring enormous benefit to the processing of hyperspectral images and to other remote sensing data analysis because labelled data are often scarce in this field. We propose a method for clustering the pixels of hyperspectral images using sparse coefficients computed from a representative dictionary as features. We show empirically that the proposed method works more effectively than clustering on the original pixels. We also demonstrate that our approach, in certain circumstances, outperforms the clustering results of features extracted using principal component analysis and non-negative matrix factorisation. Furthermore, our method is suitable for applications in repetitively clustering an ever-growing amount of high-dimensional data, which is the case when working with hyperspectral satellite imagery.

==> title_page.tex <==
\begin{titlepage}
\begin{center}
\vspace*{0.5cm}
\textsc{\large University of the Witwatersrand}\\
\includegraphics[width=0.12\textwidth]{witslogonew.png}~\\[0.2cm]
\large School of Computer Science and Applied Mathematics\\
\large Faculty of Science\\
\textsc{\Large Honours Research Report}\\[1.8cm]
% Title
\textbf{\huge {Dictionary Learning for Clustering on Hyperspectral Images}} \\[1.5cm]
% Author
\textbf{\Large Joshua Bruton} \\[7cm]
\vfill 
%Supervisor
Supervisor: Dr. Hairong Wang\\[1cm]

% Bottom of the page
{\normalsize {October 2019, Johannesburg}}
\end{center}
\end{titlepage}

